DSL-Assembly: A Robust and Safe Assembly Strategy

A reinforcement learning (RL) based method that enables the robot to accomplish the assembly-type task with safety regulations is proposed. The overall strategy consists of grasping and assembly, and this paper mainly considers the assembly strategy. Force feedback is used instead of visual feedback to perceive the shape and direction of the hole in this paper. Furthermore, since the emergency stop is triggered when the force output is too large, a force-based dynamic safety lock (DSL) is proposed to limit the pressing force of the robot. Finally, we train and test the robot model with a simulator and build ablation experiments to illustrate the effectiveness of our method. The models are independently tested 500 times in the simulator, and we get an 88.57% success rate with a 4mm gap. These models are transferred to the real world and deployed on a real robot. We conducted independent tests and obtained a 79.63% success rate with a 4mm gap. Simulation environments: https://github.com/0707yiliu/peg-in-hole-with-RL.

==> includes/acknowledgment.tex <==
\section*{Acknowledgment}
\label{sec:ack}

==> includes/conclusion.tex <==
\section{Conclusion and Future Works}
\vspace{-2mm}
\label{sec:conclusion}
% In this paper, a hybrid soft contact model that can online identify and switch between the reference soft contact model accordingly is proposed. The system ensures that the selected soft contact model is the most suitable one for encountered soft tissue . The ART-\uppercase\expandafter{\romannumeral 2} neural network is used to establish the hybrid soft contact model. It makes the hybrid model expandable and can quickly select a suitable soft contact model according to online measurement signals. 
% To prevent the network from expanding frequently, a drop threshold and a corresponding Euclidean distance are set. The least square method is used to identify the parameters of the model online, which allows the model could be updated online. Experiments showed that the hybrid soft contact model proposed in this paper performs better than different single soft contact models under the same conditions. New reference models can be supplemented online to enrich the hybrid soft contact model without affecting the effectiveness. 
% % Note that, this proposed method switches models in real-time, hence it is necessary to consider the sampling conditions of the control system to ensure the stability of the system, but the model only considers the force feedback in one direction.
% Note that the current hybrid model test platform only considers the force feedback in one direction. In future work, the model will use a six-degree-of-freedom manipulator. Consequently, the surgical instrument can obtain information from the six-dimensional force/torque sensor so as to obtain other force interaction information such as friction, which enhances the robustness of the model.

% \vspace{-2mm}
% \section{Acknowledgement}
% \vspace{-1mm}
% This work was supported by the National Natural Science Foundation of China with grant no. 61803103. D. Wu is part of the ATLAS project that received funding from the European Union’s Horizon 2020 research and innovation program under the Marie Sklodowska-Curie grant agreement No. 813782.


==> includes/relatework.tex <==
\vspace{-5pt}
\section{Related Work and Background}
\label{sec:related works}
\subsection{Assembly-type Task}
% Assembly-type tasks, such as peg insertion and screw tightening, have progressed considerably in the last few years due to the daily demands. 
Assembly policies \cite{pih-measurement1} typically rely exclusively on visual feedback, tactile feedback, and force control, and assume sufficiently accurate state estimates for the process. 

Some studies adapt to objects with specific shapes. 
\cite{pih-vision-shape1} used a hybrid vision model to estimate the assembly error and improve the assembly accuracy, making the model applicable to the assembly of cylinders. 
\cite{pih-shape1} explored the use of robots to autonomously assemble parts with different textures but with no change in shape. 
\cite{pih-vision-shape2} observed the robot and the hole position to complete the insertion of the USB port through the visual servo. 
However, these models cannot be adapted for other shapes of the grasped object and do not allow the robot to interact well with the environment in the case of visual observation only. 

There are some studies that accomplish the task through tactile and force perception, such as blind search alignment based on spiral force \cite{pih-forcemulshape1}, alignment based on spherical tree representation to simulate contact forces \cite{pih-forcemulshape2}, and alignment based on controllers with 6-degree-of-freedom (DoF) F/T sensors \cite{pih-forcemulshape3}. These force-based methods can be adapted to different shapes, but are inefficient and require elaborate settings for the environment and model parameters. We refer to the efficacy of force perception, including promoting the robot to make gentle contact with objects, the assurance of safety, and the ability to explore the target hole.

\subsection{Machine Learning for Assembly}
\label{sec:sec:MLfA}
Machine Learning has received attention recently in robot manipulation tasks. 
\cite{ml-force1} proposed the contact-state classification model based on a support vector machine, which can be applied to hole positions with different inclination angles. 
\cite{ml-vision1} utilized a convolutional neural network to obtain the precise position of the hole. 
These methods take into account the compliance of the robot, i.e., not colliding too violently with the environment, yet do not have the generality that machine learning methods have. 

A series of learning-based methods are used in the control loop of the system, for instance,
\cite{ml-pih1} constructed a behavior tree architecture and inserts the results into a genetic algorithm to solve the robot assembly problem. 
But a large amount of data is needed to support the model, and RL can use simulation to complete the data generation. The standard RL setting that consists of an agent interacting with the environment is considered in this paper. The environment is built as a Markov decision process with one state space $\mathcal{S}$, one action set $\mathcal{A}$. At each time step, the agent obtains the observation $s_t$, then takes one action $a_t$, and obtains one reward $r_t$.
Some studies \cite{ml-rl-impedance1, ml-rl-impedance3} use RL algorithms to adjust the matrix of the controller.
\cite{ml-rl-pih1} learned robot skill parameters through simulation based on different types of algorithms so that both simulated and real robots have assembly skills.
\cite{ml-encode-vision1} empowered the robot with multimodal representation and set up motion encoders to control the robot based on the Trust Region Policy Optimization (TRPO) \cite{TRPO} algorithm. 
\cite{ml-encode-vision2} deployed the gradient-based Proximal Policy Optimization (PPO) \cite{PPO} algorithm to robot motion control in automotive assembly tasks. These works have good robustness by utilizing a variety of sensors and adjusting the robot's motion trajectory according to the rotation of the object, they can cope with the assembly of different shapes of objects, but no restrictions are set on the robot's motion trajectory and they allow the robot's end-effector to execute its exploration on the surface of the object.
% Most of the above RL-based methods have to simulate the task in a simulator and train the policy, which cannot be fully reproduced on the real robot as the simulator cannot fully simulate the real environment.
% \cite{rl-s2r1} reduced the gap and accomplished the assembly task by a priori making the simulator model similar to the dynamics model of the real robot. 
% In this paper, we construct motion constraints to ensure the safety of the system and focus mainly on the motion state of the robot's end-effector (EEF) to simplify the difficulty of transferring from simulation to reality.
We construct motion constraints to ensure the system's safety and focus mainly on the motion state of the robot to simplify the difficulty of transferring from simulation to reality. 


